Serialized Interacting Mixed Membership Stochastic Block Model

Last years have seen a regain of interest for the use of stochastic block modeling (SBM) in recommender systems. These models are seen as a flexible alternative to tensor decomposition techniques that are able to handle labeled data. Recent works proposed to tackle discrete recommendation problems via SBMs by considering larger contexts as input data and by adding second order interactions between contexts' related elements. In this work, we show that these models are all special cases of a single global framework: the Serialized Interacting Mixed membership Stochastic Block Model (SIMSBM). It allows to model an arbitrarily large context as well as an arbitrarily high order of interactions. We demonstrate that SIMSBM generalizes several recent SBM-based baselines. Besides, we demonstrate that our formulation allows for an increased predictive power on six real-world datasets.

==> Table_results.tex <==
\begin{table*}
    \caption{Results for every dataset presented. The letters in superscript represent the model SIMSBM generalizes in this particular configuration (MMSBM \cite{Airoldi2008MMSBM}=$^{\text{a}}$; Bi-MMSBM \cite{Antonia2016AccurateAndScalableRS}=$^{\text{b}}$; IMMSBM \cite{Poux2021IMMSBM}=$^{\text{c}}$; T-MBM \cite{Tarres2019TMBM}=$^{\text{d}}$). Overall, we see that our formulation allows to improve results on every dataset.}
    \label{table-res}
	\centering
	\begin{tabular}{|l|l|l|S|S|S|S|S|S|S}

		\cline{1-9}
		& & & \text{F1} & \text{P@1} & \text{AUCROC} & \text{AUCPR} & \text{RankAvgPrec} & \text{CovErrNorm} \\ 

		\cline{2-9}
		\multirow{8}{*}{\rotatebox[origin=c]{90}{\footnotesize \text{\textbf{MrBanks 1}}}}

		& \multirow{8}{*}{\rotatebox[origin=c]{90}{\footnotesize \text{\textbf{Ply, Sit (3), Gen, Age}}}}
		& SIMSBM(1,1,1,1) &  \num{ 0.7124 +- 0.0002 } &  \num{ 0.6549 +- 0.0003 } &  \num{ 0.7071 +- 0.0002 } &  \num{ 0.7141 +- 0.0003 } &  \num{ 0.8274 +- 0.0001 } &  \num{ 0.1726 +- 0.0001 } \\ 
		& & SIMSBM(1,2,1,1) &  \num{ 0.7107 +- 0.0002 } &  \num{ 0.6696 +- 0.0005 } &  \num{ 0.7120 +- 0.0004 } &  \num{ 0.7158 +- 0.0005 } &  \num{ 0.8348 +- 0.0003 } &  \num{ 0.1652 +- 0.0003 } \\ 
		& & SIMSBM(1,3,1,1) &  \maxf{ \num{ 0.7348 +- 0.0002 } } & \maxf{ \num{ 0.7172 +- 0.0005 } } & \maxf{ \num{ 0.7610 +- 0.0004 } } & \maxf{ \num{ 0.7646 +- 0.0004 } } & \maxf{ \num{ 0.8586 +- 0.0003 } } & \maxf{ \num{ 0.1414 +- 0.0003 } } \\ 
		& & TF &  \num{ 0.6795 } &  \num{ 0.6037 } &  \num{ 0.4702 } &  \num{ 0.4967 } &  \num{ 0.8019 } &  \num{ 0.1981 } \\ 
		& & NMF &  \num{ 0.7178 } &  \num{ 0.6976 } &  \num{ 0.7232 } &  \num{ 0.7182 } &  \num{ 0.8409 } &  \num{ 0.1591 } \\ 
		& & KNN &  \num{ 0.7023 } &  \num{ 0.6648 } &  \num{ 0.6859 } &  \num{ 0.6623 } &  \num{ 0.8324 } &  \num{ 0.1676 } \\ 
		& & NB &  \num{ 0.6867 } &  \num{ 0.6382 } &  \num{ 0.6323 } &  \num{ 0.6250 } &  \num{ 0.8191 } &  \num{ 0.1809 } \\ 
		& & BL &  \num{ 0.6795 } &  \num{ 0.6037 } &  \num{ 0.5000 } &  \num{ 0.5215 } &  \num{ 0.8019 } &  \num{ 0.1981 } \\ 

		\cline{1-9}
		
		\multirow{8}{*}{\rotatebox[origin=c]{90}{\footnotesize \text{\textbf{MrBanks 2}}}}

		& \multirow{8}{*}{\rotatebox[origin=c]{90}{\footnotesize \text{\textbf{ Ply, Sit (3) }}}}
		& SIMSBM(1,1) &  \num{ 0.7032 +- 0.0001 } &  \num{ 0.6700 +- 0.0003 } &  \num{ 0.7049 +- 0.0002 } &  \num{ 0.7018 +- 0.0002 } &  \num{ 0.8350 +- 0.0002 } &  \num{ 0.1650 +- 0.0002 } \\ 
		& & SIMSBM(1,2) &  \num{ 0.7032 +- 0.0002 } &  \num{ 0.6679 +- 0.0005 } &  \num{ 0.7028 +- 0.0004 } &  \num{ 0.7010 +- 0.0004 } &  \num{ 0.8340 +- 0.0003 } &  \num{ 0.1660 +- 0.0003 } \\ 
		& & SIMSBM(1,3) & \maxf{ \num{ 0.7290 +- 0.0003 } } & \maxf{ \num{ 0.7067 +- 0.0006 } } & \maxf{ \num{ 0.7547 +- 0.0005 } } & \maxf{ \num{ 0.7530 +- 0.0006 } } & \maxf{ \num{ 0.8533 +- 0.0003 } } & \maxf{ \num{ 0.1467 +- 0.0003 } } \\ 
		& & TF &  \num{ 0.6775 } &  \num{ 0.5953 } &  \num{ 0.5054 } &  \num{ 0.5259 } &  \num{ 0.7976 } &  \num{ 0.2024 } \\ 
		& & NMF &  \num{ 0.7137 } &  \num{ 0.6908 } &  \num{ 0.7246 } &  \num{ 0.7128 } &  \num{ 0.8397 } &  \num{ 0.1603 } \\ 
		& & KNN &  \num{ 0.7100 } &  \num{ 0.6699 } &  \num{ 0.7126 } &  \num{ 0.6856 } &  \num{ 0.8349 } &  \num{ 0.1651 } \\ 
		& & NB &  \num{ 0.6802 } &  \num{ 0.6512 } &  \num{ 0.6329 } &  \num{ 0.6225 } &  \num{ 0.8256 } &  \num{ 0.1744 } \\ 
		& & BL &  \num{ 0.6775 } &  \num{ 0.5953 } &  \num{ 0.5000 } &  \num{ 0.5181 } &  \num{ 0.7976 } &  \num{ 0.2024 } \\ 

		\cline{1-9}
		
		\multirow{8}{*}{\rotatebox[origin=c]{90}{\footnotesize \text{\textbf{Spotify}}}}

		& \multirow{8}{*}{\rotatebox[origin=c]{90}{\footnotesize \text{\textbf{ Artists (3)}}}}
		& SIMSBM(1) &  \num{ 0.1741 +- 0.0004 } &  \num{ 0.2155 +- 0.0007 } & \maxf{ \num{ 0.7908 +- 0.0006 } } &  \num{ 0.1603 +- 0.0003 } &  \num{ 0.3827 +- 0.0004 } &  \num{ 0.0786 +- 0.0003 } \\ 
		& & SIMSBM(2) &  \num{ 0.3156 +- 0.0005 } & \maxf{ \num{ 0.3348 +- 0.0004 } } &  \num{ 0.7661 +- 0.0005 } &  \num{ 0.2545 +- 0.0003 } & \maxf{ \num{ 0.4528 +- 0.0003 } } &  \num{ 0.0938 +- 0.0006 } \\ 
		& & SIMSBM(3) & \maxf{ \num{ 0.3243 +- 0.0004 } } &  \num{ 0.3209 +- 0.0003 } &  \num{ 0.7384 +- 0.0006 } & \maxf{ \num{ 0.2613 +- 0.0003 } } &  \num{ 0.4366 +- 0.0003 } &  \num{ 0.1079 +- 0.0007 } \\ 
		& & TF &  \num{ 0.0262 } &  \num{ 0.0042 } &  \num{ 0.4805 } &  \num{ 0.0159 } &  \num{ 0.0962 } &  \num{ 0.1550 } \\ 
		& & NMF &  \num{ 0.0371 } &  \num{ 0.0658 } &  \num{ 0.5650 } &  \num{ 0.0403 } &  \num{ 0.1762 } &  \num{ 0.2557 } \\ 
		& & KNN &  \num{ 0.3201 } &  \num{ 0.3009 } &  \num{ 0.7079 } &  \num{ 0.2400 } &  \num{ 0.3941 } &  \num{ 0.5212 } \\ 
		& & NB &  \num{ 0.0463 } &  \num{ 0.0846 } &  \num{ 0.7005 } &  \num{ 0.0576 } &  \num{ 0.2264 } & \maxf{ \num{ 0.0763 } } \\ 
		& & BL &  \num{ 0.0262 } &  \num{ 0.0532 } &  \num{ 0.5000 } &  \num{ 0.0135 } &  \num{ 0.1879 } &  \num{ 0.0969 } \\ 

		\cline{1-9}
		
		\multirow{8}{*}{\rotatebox[origin=c]{90}{\footnotesize \text{\textbf{PubMed}}}}

		& \multirow{8}{*}{\rotatebox[origin=c]{90}{\footnotesize \text{\textbf{ Symptoms (3)}}}}
		& SIMSBM(1) &  \num{ 0.2915 +- 0.0002 } &  \num{ 0.5576 +- 0.0004 } &  \num{ 0.7475 +- 0.0001 } &  \num{ 0.2658 +- 0.0001 } &  \num{ 0.4641 +- 0.0001 } &  \num{ 0.2033 +- 0.0001 } \\ 
		& & SIMSBM(2) &  \num{ 0.3127 +- 0.0001 } &  \num{ 0.5704 +- 0.0001 } &  \num{ 0.7613 +- 0.0001 } &  \num{ 0.2840 +- 0.0001 } &  \num{ 0.4838 +- 0.0000 } &  \num{ 0.1991 +- 0.0001 } \\ 
		& & SIMSBM(3) & \maxf{ \num{ 0.3219 +- 0.0001 } } & \maxf{ \num{ 0.5790 +- 0.0001 } } & \maxf{ \num{ 0.7666 +- 0.0001 } } & \maxf{ \num{ 0.2895 +- 0.0001 } } & \maxf{ \num{ 0.4937 +- 0.0001 } } & \maxf{ \num{ 0.1983 +- 0.0001 } } \\ 
		& & TF &  \num{ 0.1607 } &  \num{ 0.1003 } &  \num{ 0.5605 } &  \num{ 0.1777 } &  \num{ 0.1370 } &  \num{ 0.5118 } \\ 
		& & NMF &  \num{ 0.1606 } &  \num{ 0.0293 } &  \num{ 0.5368 } &  \num{ 0.2158 } &  \num{ 0.2321 } &  \num{ 0.2959 } \\ 
		& & KNN &  \num{ 0.2414 } &  \num{ 0.3251 } &  \num{ 0.6154 } &  \num{ 0.2324 } &  \num{ 0.2891 } &  \num{ 0.7730 } \\ 
		& & NB &  \num{ 0.2600 } &  \num{ 0.1618 } &  \num{ 0.7054 } &  \num{ 0.2389 } &  \num{ 0.2036 } &  \num{ 0.3058 } \\ 
		& & BL &  \num{ 0.1607 } &  \num{ 0.1003 } &  \num{ 0.5000 } &  \num{ 0.1026 } &  \num{ 0.2464 } &  \num{ 0.2834 } \\ 

		\cline{1-9}
		
		\multirow{7}{*}{\rotatebox[origin=c]{90}{\footnotesize \text{\textbf{Imdb 1}}}}

		& \multirow{7}{*}{\rotatebox[origin=c]{90}{\footnotesize \text{\textbf{ Usr, Cast (2) }}}}
		& SIMSBM(1,1) & \maxf{ \num{ 0.3212 +- 0.0001 } } & \maxf{ \num{ 0.2434 +- 0.0001 } } & \maxf{ \num{ 0.6265 +- 0.0001 } } & \maxf{ \num{ 0.2502 +- 0.0001 } } &  \num{ 0.4360 +- 0.0001 } &  \num{ 0.3504 +- 0.0001 } \\ 
		& & SIMSBM(1,2) & \num{ 0.2546 +- 0.0000 } &  \num{ 0.1006 +- 0.0038 } &  \num{ 0.4998 +- 0.0003 } &  \num{ 0.1509 +- 0.0001 } &  \num{ 0.2928 +- 0.0042 } &  \num{ 0.4527 +- 0.0051 } \\ 
		& & TF &  \num{ 0.2546 } &  \num{ 0.2300 } &  \num{ 0.4960 } &  \num{ 0.1485 } &  \num{ 0.4568 } &  \num{ 0.2702 } \\ 
		& & NMF &  \num{ 0.1329 } &  \num{ 0.0593 } &  \num{ 0.5007 } &  \num{ 0.1531 } &  \num{ 0.1549 } &  \num{ 0.8087 } \\ 
		& & KNN &  \num{ 0.2578 } &  \num{ 0.1899 } &  \num{ 0.5489 } &  \num{ 0.1679 } &  \num{ 0.3290 } &  \num{ 0.5328 } \\ 
		& & NB &  \num{ 0.2555 } &  \num{ 0.2351 } &  \num{ 0.5308 } &  \num{ 0.1607 } &  \maxf{ \num{ 0.4619 } } &  \maxf{ \num{ 0.2596 } } \\ 
		& & BL &  \num{ 0.2546 } &  \num{ 0.2300 } &  \num{ 0.5000 } &  \num{ 0.1508 } &  \num{ 0.4605 } &  \num{ 0.2586 } \\ 
		
		\cline{1-9}

		\multirow{6}{*}{\rotatebox[origin=c]{90}{\footnotesize \text{\textbf{Imdb 2}}}}

		& \multirow{6}{*}{\rotatebox[origin=c]{90}{\footnotesize \text{\textbf{Usr, Dir, Cast}}}}
		& SIMSBM(1,1,1) & \maxf{ \num{ 0.3896 +- 0.0001 } } & \maxf{ \num{ 0.3437 +- 0.0002 } } & \maxf{ \num{ 0.7593 +- 0.0001 } } & \maxf{ \num{ 0.3293 +- 0.0002 } } & \maxf{ \num{ 0.5705 +- 0.0001 } } & \maxf{ \num{ 0.1654 +- 0.0001 } } \\ 
		& & TF &  \num{ 0.2547 } &  \num{ 0.2238 } &  \num{ 0.5039 } &  \num{ 0.1513 } &  \num{ 0.4549 } &  \num{ 0.2636 } \\ 
		& & NMF &  \num{ 0.1127 } &  \num{ 0.0483 } &  \num{ 0.5005 } &  \num{ 0.1529 } &  \num{ 0.1406 } &  \num{ 0.8319 } \\ 
		& & KNN &  \num{ 0.2596 } &  \num{ 0.1890 } &  \num{ 0.5501 } &  \num{ 0.1681 } &  \num{ 0.3268 } &  \num{ 0.5248 } \\ 
		& & NB &  \num{ 0.2558 } &  \num{ 0.2373 } &  \num{ 0.5362 } &  \num{ 0.1617 } &  \num{ 0.4632 } &  \num{ 0.2571 } \\ 
		& & BL &  \num{ 0.2547 } &  \num{ 0.2286 } &  \num{ 0.5000 } &  \num{ 0.1507 } &  \num{ 0.4598 } &  \num{ 0.2574 } \\ 


		\cline{1-9}
	\end{tabular}
\end{table*}







\begin{table*}
	\centering
	\begin{tabular}{|l|l|l|S|S|S|S|S|S|S}

		\cline{1-9}
		& & & \text{F1} & \text{P@1} & \text{AUCROC} & \text{AUCPR} & \text{RankAvgPrec} & \text{CovErrNorm} \\ 

		\cline{1-9}
		\multirow{6}{*}{\rotatebox[origin=c]{90}{\footnotesize \text{\textbf{Imdb}}}}

		& \multirow{6}{*}{\rotatebox[origin=c]{90}{\footnotesize \text{\textbf{(1, 1)}}}}
		& SIMSBM(1,1) & \maxf{ \num{ 0.3995 +- 0.0002 } } & \maxf{ \num{ 0.3558 +- 0.0003 } } & \maxf{ \num{ 0.7665 +- 0.0001 } } & \maxf{ \num{ 0.3406 +- 0.0003 } } & \maxf{ \num{ 0.5805 +- 0.0002 } } & \maxf{ \num{ 0.1593 +- 0.0001 } } \\ 
		& & TF &  \num{ 0.2570 } &  \num{ 0.2348 } &  \num{ 0.5031 } &  \num{ 0.1541 } &  \num{ 0.4627 } &  \num{ 0.2573 } \\ 
		%& & NMF &  \num{ 0.0000 } &  \num{ 0.0226 } &  \num{ 0.5000 } &  \num{ 0.1525 } &  \num{ 0.1000 } &  \num{ 0.9000 } \\ 
		& & KNN &  \num{ 0.2668 } &  \num{ 0.2002 } &  \num{ 0.5558 } &  \num{ 0.1735 } &  \num{ 0.3308 } &  \num{ 0.4834 } \\ 
		& & NB &  \num{ 0.2585 } &  \num{ 0.2382 } &  \num{ 0.5377 } &  \num{ 0.1660 } &  \num{ 0.4664 } &  \num{ 0.2536 } \\ 
		& & BL &  \num{ 0.2570 } &  \num{ 0.2349 } &  \num{ 0.5000 } &  \num{ 0.1525 } &  \num{ 0.4647 } &  \num{ 0.2557 } \\ 

		\cline{1-9}
		
		\multirow{6}{*}{\rotatebox[origin=c]{90}{\footnotesize \text{\textbf{MrBanks}}}}

		& \multirow{6}{*}{\rotatebox[origin=c]{90}{\footnotesize \text{\textbf{(1, 1)}}}}
		& SIMSBM(1,1) & \maxf{ \num{ 0.7126 +- 0.0002 } } & \maxf{ \num{ 0.6688 +- 0.0004 } } & \maxf{ \num{ 0.7126 +- 0.0003 } } & \maxf{ \num{ 0.7180 +- 0.0004 } } & \maxf{ \num{ 0.8344 +- 0.0002 } } & \maxf{ \num{ 0.1656 +- 0.0002 } } \\ 
		& & TF &  \num{ 0.6795 } &  \num{ 0.6037 } &  \num{ 0.5176 } &  \num{ 0.5363 } &  \num{ 0.8019 } &  \num{ 0.1981 } \\ 
		& & KNN &  \num{ 0.6940 } &  \num{ 0.6433 } &  \num{ 0.6668 } &  \num{ 0.6430 } &  \num{ 0.8217 } &  \num{ 0.1783 } \\ 
		& & NB &  \num{ 0.6795 } &  \num{ 0.6037 } &  \num{ 0.5907 } &  \num{ 0.5822 } &  \num{ 0.8019 } &  \num{ 0.1981 } \\ 
		& & BL &  \num{ 0.6795 } &  \num{ 0.6037 } &  \num{ 0.5000 } &  \num{ 0.5215 } &  \num{ 0.8019 } &  \num{ 0.1981 } \\ 

		\cline{1-9}
	\end{tabular}
\end{table*}



